The Ladder and Readout Cables of Intermediate Silicon Strip Detector for sPHENIX

A new silicon-strip-type detector was developed for precise charged-particle tracking in the central rapidity region of heavy ion collisions. A new detector and collaboration at the Relativistic Heavy Ion Collider at Brookhaven National Laboratory is sPHENIX, which is a major upgrade of the PHENIX detector. The intermediate tracker (INTT) is part of the advanced tracking system of the sPHENIX detector complex together with a CMOS monolithic-active-pixel-sensor based silicon-pixel vertex detector, a time-projection chamber, and a micromegas-based detector. The INTT detector is barrel shaped and comprises 56 silicon ladders. Two different types of strip sensors of 78~$\mu m$ pitch and 320~$\mu m$ thick are mounted on each half of a silicon ladder. Each strip sensor is segmented into 8$\times$2 and 5$\times$2 blocks with lengths of 16 and 20 mm. Strips are read out with a silicon strip-readout (FPHX) chip. In order to transmit massive data from the FPHX to the down stream readout electronics card (ROC), a series of long and high speed readout cables were developed. This document focuses on the silicon ladder, the readout cables, and the ROC of the INTT. The radiation hardness is studied for some parts of the INTT devices in the last part of this document, since the INTT employed some materials from the technology frontier of the industry whose radiation hardness is not necessarily well known.

==> INTT_Reference.tex <==
%% Loading bibliography style file
%\bibliographystyle{model1-num-names}
\bibliographystyle{cas-model2-names}%\bibliography{}
\begin{thebibliography}{00}

\bibitem{sPHENIX_CDR} An upgrade concept from the PHENIX collaboration, arXiv:1207.6378v2 (2012).

\bibitem{sPHENIX_TDR} Technical Design Report of sPHENIX (2019),  https://indico.bnl.gov/event/7081/

\bibitem{PHENIX} K. Adcox {\it et al.}, Nucl. Instr. and Meth. in Physics Research Section {\bf A 499} (2003) 469. 

\bibitem{RBRCworkshop} R.~Belmont, {\it et al.}, Predictions for the sPHENIX physics program, Nucl. Phys. {\bf A 1043} (2024) 122821.

\bibitem{TPOT} S. Aune {\it et al.}, Nucl. Instr. and Meth. in Physics Research {\bf A 1066} (2024) 169615.

\bibitem{BaBar} B. Aubert {\it et al.}, Nucl. Instr. and Meth. in Physics Research {\bf A 479} (2002) 1.

\bibitem{FVTX_NIM} C. Aidala {\it et al.}, Nucl. Instr. and Meth. in Physics Research {\bf A 755} (2014) 44.

%%%%%% Silicon %%%%%%
\bibitem{SiliconHPK} Hamamatsu Photonics K.K., model S14629-01 data sheet.

\bibitem{FPHX_NIM} J.S.~Kapustinsky, Nucl. Instr. and Meth. in Physics Research {\bf A 617} (2010) 546.

\bibitem{FPHX} T.~Zimmerman and J.~Hoff, "FPHX Chip Documentation", Fermilab (2009).

%%%%%% Stave %%%%%%%
\bibitem{T700C} Toray carbon fibers, TORAYCA T700 Data sheet.

\bibitem{NT91500-520S} Nippon Graphite Fiber Corporation, Granoc PREPREG NT91500-520S Technical data. 

\bibitem{Rohacell} Evonik Industries AG, Rohacelll IG-F data sheet.

\bibitem{PEEK} Mitsubishi Chemical Advanced Materials, Ketron CA30 PEEK data sheet. 

\bibitem{EA9396} The Henkel Corporation, LOCTITE EA 9396 AERO Technical process bulletin. 

\bibitem{EP75-1} MasterBond, EP75-1 Technical data sheet.

%%%%% Ladder Assembly & X/X0 %%%%%%%%
\bibitem{SilverEpoxy} The Henkel Corporation, LOCTITE ABLESTIC 2902 Technical data sheet.

\bibitem{TC-2810} 3M, Thermally conductive epoxy adhesive TC-2810 Technical data (2018). 

%%%% BEX %%%%%
\bibitem{BEX} T. Kondo {\it et al.}, Development of Long and High-Density Flexible Printed Circuits, Journal of The Japan Institute of Electronics Packaging, E21-007-1, {\bf 15} (2022).

\bibitem{FeliosLCP} Panasonic Industry Co., Ltd., FELIOS data sheet. 

%\bibitem{Arisawa} Arisawa Manufacturing co. ltd., low dielectric constant bonding sheet A26R series.

%%%% Conversion Cable %%%%%
\bibitem{IPEX} I-PEX Inc., CABLINE-UX II data sheet.

%\bibitem{AosenHarness} Aosen Coaxial cable Product Specification SP-10005-027A coaxial cable data sheet.

\bibitem{CopperResitance} R.~A.~Matula, Electrical resistivity of copper, gold, palladium, and silver, Journal of Physical and Chemical Reference Data {\bf 8} (1979) 1147.

\bibitem{OSTI} L. Whinnery {\it et al.}, "Radiation Effects on Teflon Wires", SAND2017-9103C, 656517 (2017).

\bibitem{TLK2711} A. Aloisio and R. Giordano, "Results of the TLK2711-A Radiation Tolerance Tests", XVI SuperB Workshop, Frascati, Italy (2011).


%\bio{pic1}
% Here goes the biography details.


\end{thebibliography}
